Deficiency of Large Language Models in Finance: An Empirical Examination of Hallucination

The hallucination issue is recognized as a fundamental deficiency of large language models (LLMs), especially when applied to fields such as finance, education, and law. Despite the growing concerns, there has been a lack of empirical investigation. In this paper, we provide an empirical examination of LLMs' hallucination behaviors in financial tasks. First, we empirically investigate LLM model's ability of explaining financial concepts and terminologies. Second, we assess LLM models' capacity of querying historical stock prices. Third, to alleviate the hallucination issue, we evaluate the efficacy of four practical methods, including few-shot learning, Decoding by Contrasting Layers (DoLa), the Retrieval Augmentation Generation (RAG) method and the prompt-based tool learning method for a function to generate a query command. Finally, our major finding is that off-the-shelf LLMs experience serious hallucination behaviors in financial tasks. Therefore, there is an urgent need to call for research efforts in mitigating LLMs' hallucination.

==> abandon.tex <==

\paragraph{Instruction-tuning enhances the financial Domain generalization of general language models}. In examining the data from our experiments, a clear trend emerges regarding the generalization abilities of language models in the finance domain after undergoing instruction-tuning. As detailed in Table \ref{tab:acronym} and Table \ref{long-form} , the 'Llama-2-chat' model, which is assumed to be the chat-finetuned version of the foundation model, consistently outperforms its counterpart, 'Llama-2', across various decoding methods. Notably, with the greedy decoding method, the accuracy of 'Llama-2-chat' reaches an impressive 76.0\%, a marked increase from the 57.29\% accuracy of 'Llama-2'. This trend is further corroborated by the results in Table 2, where 'Llama-2-chat' consistently scores higher on the FactScore and exhibits zero degenerations in the long-form generation task. These findings collectively highlight the immense potential of instruction-tuning in enhancing the generalization prowess of language models for finance-related tasks.




\begin{table}
    \centering
    \caption{The acronym test results for the foundation model and the chat-finetuned model. $^{\dagger}$The results with RAG applied across different decoding methods are all the same for the same model.}
    \begin{tabular}{lcc|lcc}
        \toprule
        \multicolumn{3}{c|}{Llama-2} & \multicolumn{3}{c}{Llama-2-chat} \\
        \cmidrule{1-3} \cmidrule{4-6}
        Decoding  & Method & Accuracy(\%) & Decoding &  Method & Accuracy(\%) \\
        \midrule

        $top\_p$=0.9 & Zero-Shot & 25.00 &  $top\_p$=0.9 & Zero-Shot & 73.97\\
        $top\_p$=0.7 & Zero-Shot & 34.13 &  $top\_p$=0.7 & Zero-Shot & 67.92 \\
        $top\_p$=0.5 & Zero-Shot & 46.87 &  $top\_p$=0.5 & Zero-Shot & 47.92 \\
        $top\_p$=0.3 & Zero-Shot & 52.08 &  $top\_p$=0.3 & Zero-Shot & 60.42 \\
        $top\_p$=0.1 & Zero-Shot & \textbf{59.30} &  $top\_p$=0.1 & Zero-Shot & 71.88 \\
        
        greedy &  Zero-Shot & 57.29 & greedy & Zero-Shot & \textbf{76.04} \\
        \midrule
        \textit{Any} $^{\dagger}$& RAG & 89.58   &  \textit{Any}$^{\dagger}$ & RAG & 95.83 \\
        \bottomrule
    \end{tabular}

    \label{tab:acronym}
\end{table}


         %$top\_p$=0.9 & RAG & 89.58   &  $top\_p$=0.9 & RAG & 95.83 \\
         %$top\_p$=0.7 & RAG &89.58    &  $top\_p$=0.7 & RAG & 95.83 \\
         %$top\_p$=0.5 & RAG & 89.58   &  $top\_p$=0.5 & RAG & 95.83 \\
         %$top\_p$=0.3 & RAG &89.58    &  $top\_p$=0.3 & RAG & 95.83 \\
         %$top\_p$=0.1 & RAG & 89.58   &  $top\_p$=0.1 & RAG & 95.83 \\
        %greedy & RAG & 89.58    & greedy & RAG & 95.83 \\


\begin{table}[h]
    \centering
    \caption{The results of the long-form generation task. $^{*}$We used the FactScore \cite{min2023factscore} with the GPT-4 and the retrieval from the default wikipedia database as our metric. $^{\dagger}$These columms indicates the percent of degenerations. $^{\ddagger}$ The results with RAG applied across different decoding methods are all the same for the same model.} 
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        & \multicolumn{3}{c|}{Llama-2} & \multicolumn{3}{c|}{Llama-2-chat} \\
        \cline{2-7}
        Setup & \# facts & FactSc.$^{*}$ (\%) & degen.$^{\dagger}$ (\%) & \# facts & FactSc.$^{*}$ (\%) & degen.$^{\dagger}$ (\%) \\
        \hline

        0.9 & 22.80 & 36.15 & 2.27 & 33.91 & 53.57 & 0.00 \\
       % \hline
        0.7 & 25.82 & 41.09 & 1.24 & 34.84 & 56.57 & 0.00 \\
       % \hline

        0.5 & 25.78 & 46.98 & 0.61 & DD & DD & DD \\
        %\hline
        0.3 & 26.93 & 51.94 & 0.00 & DD & DD & DD \\
        %\hline

        0.1 & 24.42 & 51.08 & 0.00 & DD & DD & DD \\
        %\hline
        greedy & 24.56 & 49.88 & 0.00 & 32.29 & 64.68 & 0.00 \\
        \hline
        RAG$^{\ddagger}$ & 26.92 & 75.07 & 4.40 & 17.49 & \textbf{90.48} & 0.00 \\

        %0.9+RAG & 26.92 & 75.07 & 4.40 & 17.49 & 90.48 & 0.00 \\
        %\hline
        %0.7+RAG & 26.92 & 75.07 & 4.40 & 17.49 & 90.48 & 0.00 \\
        %\hline
        %0.5+RAG & 26.92 & 75.07 & 4.40 & 17.49 & 90.48 & 0.00 \\
        %\hline
        %0.3+RAG & 26.92 & 75.07 & 4.40 & 17.49 & 90.48 & 0.00 \\
        %\hline
        %0.1+RAG & 26.92 & 75.07 & 4.40 & 17.49 & 90.48 & 0.00 \\
        %\hline
        %greedy+RAG & 26.92 & 75.07 & 4.40 & 17.49 & 90.48 & 0.00 \\
        \hline
    \end{tabular}

    \label{long-form}
\end{table}

\begin{table}[h]
    \centering
    \caption{The comparative performance of Llama-2 and Llama-2-chat models, with and without a specialized tool, across various decoding strategies. The metrics capture the mean absolute error (MAE) between the ground truth and the predicted prices, the percentage of valid answers (valid), the percentage of answers that the integer parts are correct (int\_correct), and the overall accuracy.}
    \begin{tabular}{|l|l|l|l|l|l|}
        \hline
        Model & Decoding & MAE (\$) & Valid (\%)  & int\_correct (\%)  & Accuracy (\%) \\
        \hline
        \multirow{8}{*}{Llama-2} & $top\_p$=0.9 & 6,307.97 & 100.00 & 1.09 & 0.00 \\
        & $top\_p$=0.7 & 6,378.03 & 100.00 & 1.40 & 0.00 \\
        & $top\_p$=0.5 & 6,360.40 & 100.00 & 0.91 & 0.00 \\
        & $top\_p$=0.3 & 6,359.07 & 100.00 & 0.91 & 0.00 \\
        & $top\_p$=0.1 & 6,357.67 & 100.00 & 1.99 & 0.00 \\
        & Greedy & 6,368.84 & 100.00 & 1.63 & 0.00 \\
        \hline
        \multirow{8}{*}{Llama-2 + tool} & $top\_p$=0.9 & - & - & - & 35.51 \\
        & $top\_p$=0.7 & - & - & - & 55.25 \\
        & $top\_p$=0.5 & - & - & - & 97.82 \\
        & $top\_p$=0.3 & - & - & - & 100.00 \\
        & $top\_p$=0.1 & - & - & - & 100.00 \\
        & Greedy & - & - & - & 100.00 \\
        
        \hline
        
        \multirow{8}{*}{Llama-2-chat} & $top\_p$=0.9 & 6,613.41 & 98.55 & 1.09 & 0.00 \\
        & $top\_p$=0.7 & 6,406.50 & 98.19 & 1.26 & 0.00 \\
        & $top\_p$=0.5 & 6,512.23 & 97.83 & 1.27 & 0.00 \\
        & $top\_p$=0.3 & 6,385.21 & 99.82 & 1.81  & 0.00 \\
        & $top\_p$=0.1 & 6,384.39 & 99.82 & 2.72 & 0.00 \\
        & Greedy & 6,380.51 & 99.64 & 2.53 & 0.00 \\
        
        \hline
        
        \multirow{8}{*}{Llama-2-chat + tool} & $top\_p$=0.9 & - & - & - & 90.94 \\
        & $top\_p$=0.7 & - & - & - & 96.38 \\
        & $top\_p$=0.5 & - & - & - & 100.00 \\
        & $top\_p$=0.3 & - & - & - & 100.00 \\
        & $top\_p$=0.1 & - & - & - & 100.00 \\
        & Greedy & - & - & - & 100.00 \\
        \hline

    \end{tabular}

    \label{tab:tooluse}
\end{table}

\hfill
    \small
    \hspace{0.2in}
    \begin{minipage}{0.52\linewidth}
        \centering
        \caption{Results of the financial term explanation task. $^{*}$F.S. stands for FactScore \cite{min2023factscore}.}
        %\small
        \begin{tabular}{lccccc}
            \toprule
            Model         & Method    & \# Facts & $^{*}$F.S. (\%) \\
            \midrule
            Llama2-7B     & Direct & 26.93 & 51.94 \\
            Llama2-7B-chat& Direct & 32.29          & 64.68 \\
            GPT3.5-turbo  & Direct & 57.88          & 78.54 \\
            GPT4           & Direct & 65.88        & 81.11 \\
            Llama2-7B     & RAG       & 26.92       & 75.07 \\
            Llama2-7B-chat& RAG      & 17.49          & \textbf{90.48} \\

            \bottomrule
        \end{tabular}
        \label{tab:long-form_whole}
    \end{minipage}

\begin{table*}
    %\begin{minipage}{0.46\linewidth}
        \centering
        \caption{Results of the acronym recognition task and terminology explanation task.}
        \begin{tabular}{lcccc}
            \toprule
            &  &\multicolumn{1}{c}{Acronym} & \multicolumn{2}{c}{Term explanation} \\
            Model  & Method    & (acc.)  & (\# facts) & (FS) \\
            \midrule
            \multicolumn{5}{c}{\textit{Baselines}} \\
            Llama2-7B     & Zero-Shot & 59.30 & 26.93 & 51.94\\
            Llama2-7B-chat& Zero-Shot  & 76.04 & 32.29   & 64.68\\
            Llama2-13B     & Zero-Shot & 73.96 & 28.45 & 56.08  \\
            Llama2-13B-chat& Zero-Shot  & 75.00 & 23.77   & 66.72 \\
            PIXIU$_{7B}$& Zero-Shot  &  30.21 & -   & - \\
            GPT3.5-turbo  & Zero-Shot  & 85.42 & 57.88   & 78.54\\
            GPT4           & Zero-Shot & 90.63 & 65.88   & 81.11\\
            Llama2-7B     & Few-Shot & 58.29& 14.67 & 51.60\\
            Llama2-7B-chat& Few-Shot  & 77.08 & 17.43 & 67.02\\
            Llama2-13B     & Few-Shot & 58.33 & 14.54 & 63.28\\
            Llama2-13B-chat& Few-Shot  & 76.04 & 16.23 & 67.97\\
            PIXIU$_{7B}$& Few-Shot  &  42.70 & -   & - \\
            \midrule
            \multicolumn{5}{c}{\textit{Decoding}} \\
            Llama2-7B    & Dola & 75.00 & 33.82 & 56.39 \\
            Llama2-7B-chat& Dola & 80.21& 34.74 & 65.42 \\ 
            Llama2-13B    & Dola & 76.45 & 35.42 & 67.06 \\
            Llama2-13B-chat& Dola & 82.67 & 38.27 & 67.50 \\ 
            \midrule
            \multicolumn{5}{c}{\textit{Methods with Retrieval}} \\
            Llama2-7B     & RAG   & 89.58 & 26.92  & 75.07\\
            Llama2-7B-chat& RAG   & 95.83 & 17.49  &  90.48\\
            Llama2-13B     & RAG   & 90.42 & 27.34  & 78.56\\
            Llama2-13B-chat& RAG   & \textbf{96.42} & 18.31  & \textbf{90.67}  \\
            \bottomrule
        \end{tabular}
        \label{tab:reference}
    %\end{minipage}%
\end{table*}


The challenge of ensuring that LLMs produce accurate and reliable information in the financial sector is multifaceted. Firstly, financial data is highly dynamic, with new information continuously flowing in from global markets, making it imperative for models to be updated and to reason over current data. Secondly, the intricacy and specificity of financial jargon pose the risk of misinterpretation, especially when general-purpose LLMs, not fine-tuned on financial data, are deployed. Furthermore, the high stakes associated with financial decisions mean that even minor errors can cascade into significant setbacks. There is also the ethical dimension to consider: stakeholders in the financial sector—be it investors, analysts, or everyday individuals—deserve transparent and reliable tools to aid their decision-making. With these challenges at hand, there is a pressing need to develop methodologies that not only harness the capabilities of LLMs in finance but also rigorously address their limitations, ensuring their outputs are not just plausible-sounding, but firmly rooted in accuracy and reliability.





\paragraph{Lower top\_p leads to less hallucinations}

\paragraph{}

==> uncertainty.tex <==

\begin{table*}
    %\begin{minipage}{0.46\linewidth}
        \centering
        \caption{Results of the uncertainty-based metrics performance on acronym recognition task and terminology explanation task.}
        \begin{tabular}{lcccccc}
            \toprule
             &\multicolumn{1}{c}{Acronym} & \multicolumn{4}{c}{Term explanation} \\
            Model     & (acc.)  & (NLL-ngram)$\downarrow$ & (BERTScore)$\downarrow$& (QA)$\downarrow$ & (NLI)$\downarrow$ \\
            \midrule
            \multicolumn{5}{c}{\textit{Zero-shot}} \\
            Llama2-7B-chat& 74.08   & - & - & - &\\
            Llama2-13B-chat& 79.59  & 4.29& 46.83& 28.14 & 25.98\\
            \midrule
            \multicolumn{5}{c}{\textit{Few-shot}} \\
            Llama2-7B    & 81.25  & 5.08 & 79.33 & 42.88 & 71.04\\
            Llama2-7B-chat& 83.08 \\
            Llama2-13B & 81.38  & 4.47 & 58.06 & 32.66 & 49.23\\
            Llama2-13B-chat& 83.46  & &&&\\
            %\midrule
            %\multicolumn{6}{c}{\textit{Few-shot + Dola decoding}} \\
            %Llama2-7B    &  & 75.00 & - & -\\
            %Llama2-7B-chat&  & 80.21& - & - \\ 
            %Llama2-13B    &  & - & - & -\\
            %Llama2-13B-chat&  & - & - & - \\ 
            %\midrule
            %\multicolumn{6}{c}{\textit{RAG}} \\
            %Llama2-7B     &    & 89.58 & 26.92  & 75.07\\
            %Llama2-7B-chat&    & 95.83 & 17.49  &  90.48\\
            %Llama2-13B     &    & 90.42 & 27.34  & 78.56\\
            %Llama2-13B-chat&    & \textbf{96.42} & 18.31  & \textbf{90.67}  \\
            \bottomrule
        \end{tabular}
        \label{tab:uncertainty}
    %\end{minipage}%
\end{table*}



\revision{\textbf{Uncertainty-based metric}. We generate 6 extra samples by nucleus decoding~\cite{holtzman2019curious} with $top\_p=0.9$, and count one acronym as \textit{correctly recognized} if more than half of the samples (i.e. $>3$) matches the predicted full name using the same EXACT string match rule.}

\revision{\textbf{Uncertainty-based metric}. To evaluate the effectiveness of uncertainty-based hallucination metrics for black-box LLMs, we generate 6 samples by nucleus decoding~\cite{holtzman2019curious} with $top\_p=0.9$ and measure their consistency. We utilize the three variants of SelfCheckGPT~\cite{manakul2023selfcheckgpt}: n-gram, multiple-choice question answering generation (MQAG), and Natural Language Inference (NLI) in this task.}
